Permissionless Blockchains and Secure Logging

The blockchain technology enables mutually untrusting participants to reach consensus on the state of a distributed and decentralized ledger (called a blockchain) in a permissionless setting. The consensus protocol of the blockchain imposes a unified view of the system state over the global network, and once a block is stable in the blockchain, its data is visible to all users and cannot be retrospectively modified or removed. Due to these properties, the blockchain technology is regarded as a general consensus infrastructure and based on which a variety of systems have been built. This article presents a study and survey of permissionless blockchain systems in the context of secure logging. We postulate the most essential properties required by a secure logging system and by considering a wide range of applications, we give insights into how the blockchain technology matches these requirements. Based on the survey, we motivate related research perspectives and challenges for blockchain-based secure logging systems, and we highlight potential solutions to some specific problems.

==> sec/analysis.tex <==
Analysis
- Overhead (computation and communication)
- Practicality
- Security analysis
Evaluation
- Compare with related work!
- Deployment issues (legacy issues?)



==> sec/overview.tex <==
Describe approach
- Repeatable, specific description
- Provide intuition, key idea
- State what the problem is that you want to address in that section
- Describe all parts of life cycle: setup, run, maintenance, etc.
- Explain with an example (together with the intuition and
  description, the scheme should have been explained 3 times from
  different perspectives)
- Did we really fully explore the design space?
  - Why are simpler solutions inappropriate?
  - Explore design alternatives!
  - Provide intuition on why certain design choices were taken, why alternatives were rejected
  - Describe a strawman approach, show why it's inadequate

A high level description is presented in \autoref{fig:overview}.
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.7\linewidth]{fig/overview}
  \caption{A high-level overview of the protocol.}
  \label{fig:overview}
\end{figure}


==> sec/pre.tex <==
Background
Problem Definition
- Clear and concise problem formulation
- Present specific quality metric for evaluation
Attacker Model
Assumptions

The notation used throughout the paper is presented in \autoref{tab:notation}
\begin{table}[h!]
\begin{center}
% \renewcommand*{\arraystretch}{1.25}
    \begin{tabular}{ll}
$\{msg\}_A$ & denotes the message $msg$ digitally signed by $A$, \\
$h(.)$ & is a cryptographic hash function, \\
$\|$ & is the string concatenation, \\
$r\xleftarrow{R}S$ & denotes that $r$ is an element randomly selected from the set $S$,\\
$\{0,1\}^n$ & is a set of all $n$-bit long strings,\\
$t_x$ & is a Unix timestamp expressed in seconds. \\
\end{tabular}
\end{center}
    \caption{Notation used throughout the paper.}
    \label{tab:notation}
\end{table}


==> sec/related.tex <==
Secure Logging systems based on blockchain technologies

\subsection{Commitcoin}
Commitcoin~\cite{Clark12commitcoin} is a timestamped commitment scheme
based on Bitcoin. When the commitment is opened, anyone can be convinced that the commitment
was made before certain time.

Assume that Alice is a Bitcoin user with a key pair $(sk, pk)$ who wants to
make a commitment of message $m$. Alice first computes the commitment
$c = \mathsf{Comm}(m, r)$, and derives a new key pair $(sk', pk')$ with the private
key $sk' = c$. Then Alice signs a Bitcoin transaction $\tau_1 = \langle pk \rightarrow pk', 2 \rangle$
which sends 2 BTC from $pk$ to $pk'$ with randomness
$\rho$: $\sigma_1 = \mathsf{Sign}_{sk}(\tau_1, \rho)$.
Alice signs another transaction $\tau_2 = \langle pk' \rightarrow pk, 1 \rangle$ with
randomness $\rho'$: $\sigma_2 = \mathsf{Sign}_{sk'}(\tau_2, \rho')$.
The signed transactions are broadcast to the Bitcoin network to be included
in the public blockchain, which proves that Alice knows the corresponding private
keys of $pk$ and $pk'$. Alice can make the commitment publicly available by
signing a transaction $\tau_3 = \langle pk' \rightarrow pk, 1 \rangle$ returning the remaining
1 BTC back to her account with previously used randomness and broadcasting it to the Bitcoin network.
$\rho'$: $\sigma_3 = \mathsf{Sign}_{sk'}(\tau_3, \rho')$.
Note that this operation effectively leaks $sk' = c$ to the public since the
same key and randomness are used to generate the signatures $\sigma_2$ and $\sigma_3$~\cite{Clark12commitcoin}.
Finally, Alice can open the commitment by announcing $(m, r)$, and the timestamp of the
block containing $\tau_1$ indicates a rough time at which the commitment was created.

The accuracy of the timestamp of the commitment scheme
completely depends on
the accuracy of the timestamp of the Bitcoin blockchain, which is
known to be easily manipulated and unreliable~\cite{timeJacking}.
Therefore, this scheme may be not applicable in time-sensitive applications.

\subsection{Namecoin}
Namecoin is a name-value pairing log system based on Bitcoin with no centralized naming server~\cite{ali2016blockstack}. Namecoin achieves human-readability, strong ownership and decentralization for a naming log system while no previous systems can provide both theses three properties. 

In Namecoin, a user first register a name-value pair that he/she wants to record. At sometime, the user issues a transaction and attaches the record. Once this transaction is involved in the blockchain and confirmed by enough after-coming blocks, the creating operation is done. This record and owner address will be seen by every node in the blockchain network. For updating the record, the owner issues a transaction that contains the updated information.

The initial motivation for Namecoin was to create an alternate DNS-like system that replaces DNS root
servers with a blockchain for mapping domain names to DNS records. Namecoin is built based on Bitcoin, thus the accessibility, immutability and non-equivocation are preserved. The Latency of creating and updating records is capped by Bitcoin's consensus protocol, and its average time is 60 minutes. Thus, the availability is undetermined and up to the applications. The Authentication property is not achieved as it uses a pseud-anonymous address as its identity. For freshness, Namecoin can prove the order of the name-value records. However, the exact time of a record cannot be guaranteed.


\subsection{Catena}
Catena is an efficient verifiable Bitcoin-based witnessing scheme which enables thin clients to detect a log server's equivocation efficiently. To prevent equivocation, Catena log server implements a log as an OP\_RETURN transaction chain. Each Catena transaction stores exactly one statement and spends the previous Catena transaction output. Thus Catena creates a chain of statements.

In the initialization, Catena log server issues a genesis transaction, viewed as the identity of the log server, and embeds the start statement $s_0$ to the unspendable OP\_RETURN output. Then, the log server issues the first statement $s_1$ in the log by creating a new transaction that spends the genesis transaction's output and commits that first statement via an OP\_RETURN transaction output. Thus the log servers commits a chain of logs $<s_0,s_1,\cdots,s_n>$.

Unlike previous blockchain-based attempts, Catena clients check the log for non-equivocation via Simplified Payment Verification (SPV). When verifying the statements, the client first downloads all the block headers, and small Merkle membership proofs for the relevant transactions. If the block containing the Catena statement $s_i$ transaction received enough confirmation (usually 6), the log server is assumed to non-equivocated at position $i$. Catena log server's non-equivocation is based on the difficulty of double spending in Bitcoin. If a log server wants to equivocate, it has to double spend a Bitcoin transaction output.

Catena can achieve the accessibility, immutability and non-equivocation properties straight forward. As each Catena transaction need to be added to the blockchain and wait for enough confirmations, there is a latency for the new event. The availability of Catena is ambiguous and is up to the real world scenarios. Although Catena takes the pseudonymous address as their identities, it seems that the authentication can not be guaranteed. However, each Catena transaction should spend the previous transaction's output. Once the transaction is accepted by the blockchain network, peers can trace this transaction to the genesis transaction and confirm that it is generated by the Catena log server(or authorized by Catena log server). Finally, Each statement's issuing time is also relay on the timestamp of Bitcoin, which is known to be easily manipulated and unreliable~\cite{tomescu2017catena}.
Therefore, Catena only achieve the weak freshness.

%
%\subsection{Town crier}
%\psz{I don't believe that is very related}
%Town Crier (TC)~\cite{zhangCCS16}, acting as a bridge between
%on-chain application smart contracts and off-chain
%HTTPS-enabled websites, is realized by a
%combination of Intel's Software Guard Extensions (SGX)~\cite{Costan16SGX}
%and a smart-contract front end shown in Fig.~\ref{fig:tc}
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.6\linewidth]{fig/overview.pdf}
%	\caption{The architecture of Town Crier}
%	\label{fig:tc}
%\end{figure}
%
%
%
%The code executing within the SGX enclave is responsible for
%establishing a secure TLS channel with the HTTPS-enabled web
%server and faithfully returning the data required by the application
%smart contract through the front end contract.
%It is possible to conduct a remote attestation that the correct
%code was executed according to the Intel SGX technology.
%The risk of compromised HTTPS web servers is mitigated by
%employing a majority voting scheme among multiple websites
%offering the same piece of data required by the application contract.
%
%
%The main limitation of TC is that it places SGX as a centralized
%trusted party, contradicting the decentralized nature of the blockchain
%technology. Given that some recent attacks~\cite{Bulck18foreshadow} show that
%the SGX may be not as impenetrable as it is advertised, it is
%more desirable to have a decentralized authenticated data feed for
%smart contract avoiding such a centralized trusted entity which can
%be a single point of failure.


==> sec/scenarios.tex <==
Secure logging system has been served for many information systems in various forms. 

\subsection{Time Stamping Service}
Time stamping service is a rather conventional infrastructure
used to prove the existence of certain digital data
prior to a specific point in time. It can be a standalone system
or be an integral part of a larger system.

It is important to guarantee the accuracy and validity of the timing information
of data and events, since defect in the timing information, whether due to
intentional and unintentional reasons, may have significant security and financial
implications.

Hereby, we hight the freshness property,
which allows to order events (weak freshness) or even
to determine the exact time of them up to certain precision (strong freshness).




\subsection{Transparency Logs}
The security of many information infrastructures rely
heavily on authoritative information.
In a public-key infrastructure (PKI), Certificate Authorities (CA)
digitally sign certificates that bind an entity (e.g., a domain name)
to its public key. If a user accepts a wrong public key of the intended communication party,
someone who controls the corresponding secret key can effectively masquerade as
the legitimate entity, decrypt all traffics (including login credentials), and mislead the
user to flow malicious instructions~\cite{arthur2011rogue,roberts2011phony}.
Another example is the Tor anonymity network~\cite{tor2004}, where users select
secure relays provided by trusted directory servers to protect. The anonymity
can be completely compromised if the users are tricked to operate over malicious
relays controlled by attackers~\cite{attackTor}. Similar concerns arise in other situations
(e.g., software updates) where trusted authoritative information is relied on.
These security issues lead to the concept of transparency logs, which possess
the following properties~\cite{TP_log}.

\begin{enumerate}
	\item[$\bullet$]{\bf Append-only.}
	Transparency logs should be able to prove that the updated log contains
	all entries of the old version of the log.
	
	\item[$\bullet$]{\bf Non-equivocation.}
	The log server cannot present different views of the log for different users.	
\end{enumerate}

Note that the transparency is a very general concept. In particular, we have
key transparency~\cite{melara2015coniks}, binary transparency, and Google even launches its
General Transparency project~\cite{dowling2016secure}.


\subsection{Bridging Legacy Content with Blockchains}
Smart contracts, envisioned by Nick Szabo back in 1996~\cite{szabo2001smart}, are brought into reality
with the rise of the blockchain technology.
They allow untrusting parties to arrange self-enforcing agreements in a decentralized way.
The development of the Ethereum~\cite{wood2014ethereum} has inspired
countless on-chain applications based on smart contracts.
However, without a mechanism connecting the smart contracts with
the real world, their potential to revolutionize the way our society
operates would be severely suppressed.
It is not difficult to imagine what we can achieve if off-chain information (such as
stock quotes, weather data, sports results, and webpage contents, etc.) are made available
to smart contracts.


However, there are many challenges associated with realizing
such a bridging mechanism, which should fulfill the following properties.
\begin{enumerate}
	\item[$\bullet$]{\bf Decentralized.}
	The scheme should be decentralized in nature to make the most
	out of the blockchain technology. Besides the content provider, designated by contract parties, there should no other trust authorities.
	
	\item[$\bullet$]{\bf Authenticity.}
	The scheme can verify the authenticity of the data issued by the content provider.
	
	\item[$\bullet$]{\bf Accountable.}
	The scheme should make the content providers accountable, auditable, and therefore mitigates
	their malicious activities like data modification or censorship.
	
	\item[$\bullet$]{\bf Non-equivocation.}
	The scheme should make sure that the content providers cannot provides contradicting contents.
	
	\item[$\bullet$]{\bf Usability.}
	The data forwarded to blockchain should be easily parsable, and the overall scheme should be easy to
	adopt and deploy.
	
\end{enumerate}




